RealCQA: Scientific Chart Question Answering as a Test-bed for First-Order Logic

We present a comprehensive study of chart visual question-answering(QA) task, to address the challenges faced in comprehending and extracting data from chart visualizations within documents. Despite efforts to tackle this problem using synthetic charts, solutions are limited by the shortage of annotated real-world data. To fill this gap, we introduce a benchmark and dataset for chart visual QA on real-world charts, offering a systematic analysis of the task and a novel taxonomy for template-based chart question creation. Our contribution includes the introduction of a new answer type, 'list', with both ranked and unranked variations. Our study is conducted on a real-world chart dataset from scientific literature, showcasing higher visual complexity compared to other works. Our focus is on template-based QA and how it can serve as a standard for evaluating the first-order logic capabilities of models. The results of our experiments, conducted on a real-world out-of-distribution dataset, provide a robust evaluation of large-scale pre-trained models and advance the field of chart visual QA and formal logic verification for neural networks in general.

==> Sections/Figures/005_loss_heads.tex <==
\begin{figure}[ht!]
         \centering
         \includegraphics[width= \textwidth]{Sections/Figures/los_head.png}
         \caption{\scriptsize Affect of Keypoint loss. Top row shows output when trained in isolation : input chart, gaussian mask, predicted BCE heatmap, predicted MSE foreground, predicted MSE background, predicted CE foreground, predicted CE background. Bottom Row shows outputs when trained in combination, first two show the groundtruth Classification Mask and Regression Mask, rest are counterparts of top row outputs.}
         \label{fig:loss_he}
\end{figure}

==> Sections/Figures/006_ContrastiveKP.tex <==
\begin{figure}[ht!]
         \centering
         \includegraphics[width= 0.85\textwidth]{Sections/Figures/contrastive.png}
         \caption{\scriptsize Global chart vs key-point attention implementation to generate Contrastive Feature Map }
         \label{fig:contrKP}
\end{figure}

==> Sections/Figures/007_Filter_regression.tex <==
\begin{figure}[ht!]
         \centering
         \includegraphics[width= 0.85\textwidth]{Sections/Figures/fore_ground.png}
         \caption{\scriptsize Post-Processing Regression Prediction : (Top row) Input image, Thresholded islands, Points from connected components, (Middle Row) Colour Histogram over all points, All points from cc before filtering, (Bottom Row) Histogram after discarding pixels close to median color, Final points chosen for contrastive grouping.}
         \label{fig:filtereg}
\end{figure}
